DocDeshadower: Frequency-Aware Transformer for Document Shadow Removal

Shadows in scanned documents pose significant challenges for document analysis and recognition tasks due to their negative impact on visual quality and readability. Current shadow removal techniques, including traditional methods and deep learning approaches, face limitations in handling varying shadow intensities and preserving document details. To address these issues, we propose DocDeshadower, a novel multi-frequency Transformer-based model built upon the Laplacian Pyramid. By decomposing the shadow image into multiple frequency bands and employing two critical modules: the Attention-Aggregation Network for low-frequency shadow removal and the Gated Multi-scale Fusion Transformer for global refinement. DocDeshadower effectively removes shadows at different scales while preserving document content. Extensive experiments demonstrate DocDeshadower's superior performance compared to state-of-the-art methods, highlighting its potential to significantly improve document shadow removal techniques. The code is available at https://github.com/leiyingtie/DocDeshadower.

==> figtex/Ablation.tex <==
\begin{figure*}[ht] 
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/input_natiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_aannatiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_gmftnatiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_aannatiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_gmftnatiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_natiCHW01_08.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/target_natiCHW01_08.jpg}}
            \end{minipage} 
        \hfill        
    \end{minipage}
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/input_natiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_aannatiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_gmftnatiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_aannatiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_gmftnatiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_natiCHW02_04.jpg}}
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/target_natiCHW02_04.jpg}}
            \end{minipage} 
        \hfill        
    \end{minipage}
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/input_natiCHW02_08.jpg}}
            \centerline{(a) Input}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_aannatiCHW02_08.jpg}}
            \centerline{(b) w/o AAN}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_wo_gmftnatiCHW02_08.jpg}}
            \centerline{(c) w/o GMFT}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_aannatiCHW02_08.jpg}}
            \centerline{(d) U-Net+ANN}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/unet_gmftnatiCHW02_08.jpg}}
            \centerline{(e) U-Net+GMFT}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/ours_snatiCHW02_08.jpg}}
            \centerline{(f) Ours}\medskip
            \end{minipage} 
        \hfill
        \begin{minipage}[b]{0.136\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/Ablation/target_natiCHW02_08.jpg}}
            \centerline{(g) Target}\medskip
            \end{minipage} 
        \hfill        
    \end{minipage}
    \caption{
    We conduct a visual ablation study on several variants of our method. As depicted in the figure, variants (c), (d), and (e) display residual shadows in the output. Conversely, method (b) effectively eliminates particular shadows, albeit resulting in slight image blurriness. Our model, in comparison to others, demonstrates exceptional performance in terms of shadow removal.
    }
    \label{fig:ablation}
\end{figure*}



==> figtex/ref2.tex <==
\begin{figure*}[ht] 
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/input_natiCHW02_03.jpg}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/shadowformer_natiCHW02_03.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/sgshadow_natiCHW02_03.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/bedsr_natiCHW02_03.jpg}}
        \end{minipage}
        \hfill   
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/Liu_natiCHW02_03.jpg}}
        \end{minipage}  
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/ours_natiCHW02_03.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/target_natiCHW02_03.jpg}}
        \end{minipage}
    \end{minipage}
    \begin{minipage}[b]{1.0\linewidth}
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/input_natiCHW03_01.jpg}}
        \end{minipage}   
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/shadowformer_natiCHW03_01.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/sgshadow_natiCHW03_01.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/bedsr_natiCHW03_01.jpg}}
        \end{minipage}
        \hfill   
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/Liu_natiCHW03_01.jpg}}
        \end{minipage}  
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/ours_natiCHW03_01.jpg}}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.137\linewidth}
            \centering
            \centerline{\includegraphics[width=\linewidth]{figs/image/target_natiCHW03_01.jpg}}
        \end{minipage}
    \end{minipage}
    % \begin{minipage}[b]{1.0\linewidth}
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/input_natiCHW03_05.jpg}}
    %         \centerline{(a)Input}\medskip
    %     \end{minipage}   
    %     \hfill
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/shadowformer_natiCHW03_05.jpg}}
    %         \centerline{(b)ShadowFormer}\medskip
    %     \end{minipage}
    %     \hfill
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/sgshadow_natiCHW03_05.jpg}}
    %         \centerline{(c)SG-ShadowNet}\medskip
    %     \end{minipage}
    %     \hfill
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/bedsr_natiCHW03_05.jpg}}
    %         \centerline{(d)BEDSR-Net}\medskip
    %     \end{minipage}
    %     \hfill   
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/Liu_natiCHW03_05.jpg}}
    %         \centerline{(e)Liu \etal}\medskip
    %     \end{minipage}  
    %     \hfill
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/ours_natiCHW03_05.jpg}}
    %         \centerline{(f)Ours}\medskip
    %     \end{minipage}
    %     \hfill
    %     \begin{minipage}[b]{0.137\linewidth}
    %         \centering
    %         \centerline{\includegraphics[width=\linewidth]{figs/image/target_natiCHW03_05.jpg}}
    %         \centerline{(g)Target}\medskip
    %     \end{minipage}
    % \end{minipage}
    \caption{
    This figure offers a visual comparison across different Document Shadow Removal techniques applied to the Kligler dataset. As illustrated, method (b) leaves considerable shadow residue. Method (c) manages to remove shadows but at the cost of detail clarity, leading to a blurred output. Method (d) eliminates shadows but induces alterations in the color of the original details. Method (e) also removes shadows but results in a loss of detail.}
    \label{fig:ref2}
\end{figure*}


